SecFlow: Adaptive Security-Aware Workflow Management System in Multi-Cloud Environments

In this paper, we propose an architecture for a security-aware workflow management system (WfMS) we call SecFlow in answer to the recent developments of combining workflow management systems with Cloud environments and the still lacking abilities of such systems to ensure the security and privacy of cloud-based workflows. The SecFlow architecture focuses on full workflow life cycle coverage as, in addition to the existing approaches to design security-aware processes, there is a need to fill in the gap of maintaining security properties of workflows during their execution phase. To address this gap, we derive the requirements for such a security-aware WfMS and design a system architecture that meets these requirements. SecFlow integrates key functional components such as secure model construction, security-aware service selection, security violation detection, and adaptive response mechanisms while considering all potential malicious parties in multi-tenant and cloud-based WfMS.

==> figures/relatedworksTable.tex <==
\begin{tabulary}{\linewidth}{ P{0.11\linewidth}|P{0.1\linewidth}|P{0.1\linewidth}|P{0.1\linewidth}|P{0.25\linewidth}|P{0.2\linewidth}}
\toprule 
\textbf{\centering WfMS} &
\textbf{\centering Type of supported Workflow} &
 \textbf{\centering Supported Representation Model} &
 \textbf{\centering Extension} & 
 \textbf{\centering Execution Environment } & \textbf{\centering Covered Security Objectives }

		
  \\\hline
  
\cite{Wang2018}, 2018 &
Scientific&	DAG& 	-&	Cloud-based&
\begin{itemize}
  \item Data Integrity
  \item Data Confidentiality 
\end{itemize}
\\  \hline
SecDATAVIEW \cite{Mofrad2019}, 2019 &
Scientific&	DAG& 	DATAVIEW&	Execute the kernel of WfMS (the components that process confidential data) inside SGX enclaves (other components are executed on the trusted premises such as private cloud computing platforms
or the user side premise)&
\begin{itemize}
  \item 	Data/Task Integrity
  \item Data/Logic Confidentiality
\end{itemize}
\\  \hline

\cite{Kim2015}, 2015 &
Scientific&	DCG & 	Kepler&	Flexibly
arranged to run locally or on a cloud platform &
\begin{itemize}
  \item 	Data Integrity
\end{itemize}
\\  \hline


BPA-Sec4Cloud \cite{Lins2016}, 2016 &
Business&	BPMN & 	-&		Cloud-based &
\begin{itemize}
  \item 	Data Confidentiality
   \item 	Data Integrity
    \item 	Authentication
\end{itemize}
\\  \hline

\cite{Huang2019}, 2019 &
Business&	BPMN & 		jBPM4 &		Cloud-based &
\begin{itemize}
  \item 	Data/Logic Confidentiality
\end{itemize}
\\  \hline
\bottomrule 
\end{tabulary}\par 

==> figures/relatedworksTable2.tex <==
\begin{tabulary}{\linewidth}{ P{0.15\linewidth}|P{0.14\linewidth}|P{0.14\linewidth}|P{0.14\linewidth}|P{0.14\linewidth}|P{0.14\linewidth}}
\toprule 
 
\textbf{\centering WfMS} &
\textbf{\centering \cite{Wang2018}, 2018}  & \textbf{\centering SecDATAVIEW \cite{Mofrad2019}, 2019}  & \textbf{\centering  \cite{Kim2015}, 2015} & \textbf{\centering BPA-Sec4Cloud \cite{Lins2016}, 2016} & \textbf{\centering \cite{Huang2019}, 2019}  
\\  \hline

  
\textbf{ Workflow Structure Compatibility} &
Scientific  & Scientific  & Scientific  & Business  & Business  
\\  \hline



\textbf{\centering Scalability} &
Fully Scalable  &
Partially Scalable &
Partially Scalable &
Fully Scalable & 
Fully Scalable \\  \hline

 

\textbf{\centering Multi-Tenancy} &
No & No & No & No & Yes 
\\  \hline



 \textbf{\centering  Workflow Targets} &
Intermediate Data &
\makecell{  Intermediate \\ Data,\\ Task} &
Intermediate Data &
Intermediate Data &
\makecell{ Intermediate \\ Data, \\Logic } 
\\  \hline


 \textbf{\centering Considered Attackers} &
 \makecell{ Providers, \\ External \\ Attackers} &
 \makecell{ Providers, \\ External \\ Attackers} &
 External  Attackers & 
 External  Attackers & 
 The Engine Users (tenants) 
 \\  \hline



 \textbf{\centering Covered Attacks Categories} &
 \makecell{Network-based,  \\ VM-based } &  
 \makecell{Network-based,  \\ VM-based } & 
Application-based &
\makecell{ Network-based, \\Application-based } &
Application-based 
\\  \hline


 \textbf{\centering Covered Security Objectives} &
\makecell{Data Integrity, \\  Data \\ Confidentiality}  & 
\makecell{ Data/Task \\ Integrity, \\ Data/Logic \\  Confidentiality }  &
Data Integrity &
\makecell{ Data \\ Confidentiality, \\ Data Integrity,\\ Authentication} &
Data/Logic Confidentiality
\\  \hline

 \textbf{\centering Covered Phases of the Workflow Lifecycle} &
\makecell{  Execution,\\Monitoring } &
\makecell{  Execution,\\Monitoring } &
\makecell{  Execution,\\Monitoring } &
\makecell{Modeling,  \\ Deployment } &
\makecell{  Execution,\\Monitoring } 
\\  \hline

\bottomrule 
\end{tabulary}\par 

==> figures/relatedworksTable3.tex <==
\begin{tabulary}{\linewidth}{ P{0.12\linewidth}|P{0.11\linewidth}|P{0.1\linewidth}|P{0.09\linewidth}|P{0.08\linewidth}|P{0.13\linewidth}|P{0.12\linewidth}|P{0.09\linewidth}}
\toprule 
\textbf{\centering WfMS} &
\textbf{\centering Workflow Structure Compatibility} &
\textbf{\centering Supported Features} &
 \textbf{\centering  Workflow Targets} &
 \textbf{\centering Considered Attackers} & 
 \textbf{\centering Covered Attacks Categories} & 
 \textbf{\centering Covered Security Objectives} & 
 \textbf{\centering Covered Phases of the Workflow Lifecycle}
  \\\hline
  
\cite{Wang2018}, 2018 &
Scientific  &
Scalability  &
Intermediate Data &
 \makecell{ Providers, \\ External \\ Attackers} &	
 \makecell{Network-based,  \\ VM-based } & 
\makecell{Data Integrity, \\  Data \\ Confidentiality}  & 
 \makecell{Execution, \\  Monitoring}
\\  \hline

SecDATAVIEW \cite{Mofrad2019}, 2019 &
Scientific  &
Scalability (Partially Cloud-based) &
\makecell{  Intermediate \\ Data,\\ Task} &
 \makecell{ Providers, \\ External \\ Attackers} &	
 \makecell{Network-based,  \\ VM-based } & 
\makecell{ Data/Task \\ Integrity, \\ Data/Logic \\  Confidentiality }  & 
 \makecell{Execution, \\  Monitoring}
\\  \hline

\cite{Kim2015}, 2015 &
Scientific  &
Scalability &	
Intermediate Data &
External Attackers&
Application-based &
Data Integrity &
\makecell{ Execution, \\ Monitoring} 
\\  \hline


BPA-Sec4Cloud \cite{Lins2016}, 2016 &
Business  &
Scalability  &
Intermediate Data & 
External Attackers &	
\makecell{ Network-based, \\Application-based } &
\makecell{ Data \\ Confidentiality, \\ Data Integrity,\\ Authentication} &
\makecell{Modeling,  \\ Deployment } 
\\  \hline

\cite{Huang2019}, 2019 &
Business  &
\makecell{  Scalability , \\Multi-Tenancy } &
\makecell{ Intermediate \\ Data, \\Logic } &
The Engine Users (tenants) &	
Application-based &
Data/Logic Confidentiality &
\makecell{  Execution,\\Monitoring } 

\\  \hline
\bottomrule 
\end{tabulary}\par 

==> figures/relatedworksTable4.tex <==
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\begin{tabulary}{\linewidth}{ L{3cm}L{2.3cm}L{2.3cm}L{2.3cm}L{2.3cm}L{2.3cm}}
\Xhline{2\arrayrulewidth}
 
 \textbf{Feature} &
\textbf{\cite{Wang2018}, 2018}  & 
\textbf{ SecDATAVIEW \cite{Mofrad2019}, 2019}  &
\textbf{ \cite{Kim2015}, 2015} &
\textbf{BPA-Sec4Cloud \cite{Lins2016}, 2016}&
\textbf{\cite{Huang2019}, 2019}  
\\  \hline
\Xhline{2\arrayrulewidth}
  
\textbf{ Workflow Structure Compatibility} &
Scientific  & Scientific  & Scientific  & Business  & Business  
\\  \hline



\textbf{Scalability} &
Fully Scalable  &
Partially Scalable &
Partially Scalable &
Fully Scalable & 
Fully Scalable \\  \hline

 

\textbf{Multi-Tenancy} &
No & No & No & No & Yes 
\\  \hline



 \textbf{Workflow Targets} &
Intermediate Data &
  Intermediate Data, Task &
Intermediate Data &
Intermediate Data &
 Intermediate Data, Task 
\\  \hline


 \textbf{Covered Security Requirements} &
Data Integrity, Data Confidentiality & 
Data/Task Integrity, Data Confidentiality   &
Data Integrity &
Data Confidentiality, Data Integrity, Authentication &
Data Confidentiality, Task Confidentiality
\\  \hline


 \textbf{Considered Attackers} &
  Providers,  External  Attackers &
 Providers,  External Attackers &
 External  Attackers & 
 External  Attackers & 
 The Engine Users (tenants) 
 \\  \hline



 \textbf{Covered Attacks Categories} &
Network-based,   VM-based &  
Network-based, VM-based  & 
Application-based &
 Network-based, Application-based  &
Application-based 
\\  \hline



 \textbf{Covered Phases of the Workflow Lifecycle} &
  Execution, Monitoring  &
 Execution, Monitoring  &
  Execution, Monitoring  &
Modeling, Deployment &
  Execution, Monitoring  
\\  \hline

\bottomrule 
\end{tabulary}\par 

==> figures/relatedworksTable5.tex <==
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\begin{tabulary}{\linewidth}{ L{3cm}L{2.3cm}L{2.3cm}L{2.3cm}L{2.3cm}L{2.3cm}}
\Xhline{2\arrayrulewidth}
 
 \textbf{Feature} &
\textbf{\cite{Wang2018}, 2018}  & 
\textbf{ SecDATAVIEW \cite{Mofrad2019}, 2019}  &
\textbf{ \cite{Kim2015}, 2015} &
\textbf{BPA-Sec4Cloud \cite{Lins2016}, 2016}&
\textbf{\cite{Huang2019}, 2019}  
\\  \hline
\Xhline{2\arrayrulewidth}
  
\textbf{ Workflow Structure Compatibility} &
Scientific  & Scientific  & Scientific  & Business  & Business  
\\  \hline



%\textbf{Scalability} &
%Fully Scalable  &
%Partially Scalable &
%Partially Scalable &
%Fully Scalable & 
%Fully Scalable \\  \hline

 

\textbf{Multi-Tenancy} &
No & No & No & No & Yes 
\\  \hline



 \textbf{Workflow Targets} &
Intermediate Data &
  Intermediate Data, Task &
Intermediate Data &
Intermediate Data &
 Intermediate Data, Task 
\\  \hline


 \textbf{Covered Security Requirements} &
Data Integrity, Data Confidentiality & 
Data/Task Integrity, Data Confidentiality   &
Data Integrity &
Data Confidentiality, Data Integrity, Authentication &
Data Confidentiality, Task Confidentiality
\\  \hline


 \textbf{Considered Attackers} &
  Providers,  External  Attackers &
 Providers,  External Attackers &
 External  Attackers & 
 External  Attackers & 
 The Engine Users (tenants) 
 \\  \hline



 \textbf{Covered Attacks Categories} &
Network-based,   VM-based &  
Network-based, VM-based  & 
Application-based &
 Network-based, Application-based  &
Application-based 
\\  \hline



 \textbf{Covered Phases of the Workflow Lifecycle} &
  Execution, Monitoring  &
 Execution, Monitoring  &
  Execution, Monitoring  &
Modeling, Deployment &
  Execution, Monitoring  
\\  \hline

\bottomrule 
\end{tabulary}\par 

==> mypreamble.tex <==
\ProvidesPackage{mypreamble}

\usepackage{lineno,hyperref}
\usepackage{import}
\modulolinenumbers[5]

\journal{Journal of \LaTeX\ Templates}

%\User defined packages
% highlight
\usepackage{color,soul}
\DeclareRobustCommand{\hlc}[1]{{\sethlcolor{lightgray}\hl{#1}}}
% todonotes
\usepackage{todonotes}
% degree symbol
\usepackage{gensymb}
% tables
\usepackage{caption}
\usepackage{csvsimple}
\usepackage{booktabs, tabularx, wrapfig}
\usepackage{array, ltablex, multirow}
\usepackage{placeins}
\usepackage{graphicx}
\usepackage{subcaption}

\usepackage[nonumberlist,nogroupskip]{glossaries}

\setglossarystyle{super}

\hypersetup{%
  colorlinks=false,% hyperlinks will be black
  linkbordercolor=[rgb]{0.6,0.6,0.6},% hyperlink borders will be red
  pdfborderstyle={/S/U/W 1}% border style will be underline of width 1pt
}

%%%%%%%%%%%%%%%%%%%%%%%
%% Elsevier bibliography styles
%%%%%%%%%%%%%%%%%%%%%%%
%% To change the style, put a % in front of the second line of the current style and
%% remove the % from the second line of the style you would like to use.
%%%%%%%%%%%%%%%%%%%%%%%

%% Numbered
%\bibliographystyle{model1-num-names}

%% Numbered without titles
%\bibliographystyle{model1a-num-names}

%% Harvard
%\bibliographystyle{model2-names.bst}\biboptions{authoryear}

%% Vancouver numbered
%\usepackage{numcompress}\bibliographystyle{model3-num-names}

%% Vancouver name/year
%\usepackage{numcompress}\bibliographystyle{model4-names}\biboptions{authoryear}

%% APA style
%\bibliographystyle{model5-names}\biboptions{authoryear}

%% AMA style
%\usepackage{numcompress}\bibliographystyle{model6-num-names}

%% `Elsevier LaTeX' style
\bibliographystyle{elsarticle-num}
%%%%%%%%%%%%%%%%%%%%%%%

==> table1.tex <==
\begin{table*}[ht]
\caption{Possible Attacks in the Workflows}
\centering
\begin{tabular}{p{0.187\linewidth}|p{0.187\linewidth}|p{0.187\linewidth}|p{0.187\linewidth}}
\hline
Type of Attack & Related Attacks & Potential Targets in Workflow  & Implications of attacks \\
\hline
Application-based Attack & Fault injection, Inference Attack,
Account Hijacking, web service and protocol based attacks

& Fragment(group of tasks)
Data(Input/Output)
Message(Send/Receive)
Task(Code/Service), Control Flow Connector & Malicious manipulation of data,
Violation of data protection,
Denial-of-service\\

\hline

Network-based Attack &   port scanning, botnets, spoofing attacks, eavesdropping attack,the man-in-the-middle attack, and the replay attack     & Data(Input/Output)
Message(Send/Receive)
 Task(code/Service) &
Violation of data protection,
Denial-of-service
 \\
\hline


VM-based Attack & Cross VM   side channel attacks
VM creation attacks
VM migration and roll back attacks
VM scheduler based attacks(VM escape, VM hopping, etc.) &
Data(Input/Output)
Message(Send/Receive)
 Task(code/Service) & Violation of data protection
Denial-of-service  \\
\hline
\end{tabular}
\end{table*}

